A portable and high intensity 24 keV neutron source based on $^{124}$Sb-$^{9}$Be photoneutrons and an iron filter

A portable monoenergetic 24 keV neutron source based on the $^{124}$Sb-$^9$Be photoneutron reaction and an iron filter has been constructed and characterized. The coincidence of the neutron energy from SbBe and the low interaction cross-section with iron (mean free path up to 29 cm) makes pure iron specially suited to shield against gamma rays from $^{124}$Sb decays while letting through the neutrons. To increase the $^{124}$Sb activity and thus the neutron flux, a $>$1 GBq $^{124}$Sb source was produced by irradiating a natural Sb metal pellet with a high flux of thermal neutrons in a nuclear reactor. The design of the source shielding structure makes for easy transportation and deployment. A hydrogen gas proportional counter is used to characterize the neutrons emitted by the source and a NaI detector is used for gamma background characterization. At the exit opening of the neutron beam, the characterization determined the neutron flux in the energy range 20-25 keV to be 5.36$\pm$0.20 neutrons per cm$^2$ per second and the total gamma flux to be 213$\pm$6 gammas per cm$^2$ per second (numbers scaled to 1 GBq activity of the $^{124}$Sb source). A liquid scintillator detector is demonstrated to be sensitive to neutrons with incident kinetic energies from 8 to 17 keV, so it can be paired with the source as a backing detector for neutron scattering calibration experiments. This photoneutron source provides a good tool for in-situ low energy nuclear recoil calibration for dark matter experiments and coherent elastic neutrino-nucleus scattering experiments.

==> Section_text/discussion.tex <==
To be written


\begin{figure}[ht]
\includegraphics[width=0.8\linewidth]{Figures/NaI_rate.png}
\caption{\label{fig:NaI_rate} Event rate in NaI detector versus the distance to the Sb-124 source. The dotted line indicated the fitted curve with 1/(R*R) function}
\end{figure}
